Stochastic Coordinate Minimization with Progressive Precision for Stochastic Convex Optimization

A framework based on iterative coordinate minimization (CM) is developed for stochastic convex optimization. Given that exact coordinate minimization is impossible due to the unknown stochastic nature of the objective function, the crux of the proposed optimization algorithm is an optimal control of the minimization precision in each iteration. We establish the optimal precision control and the resulting order-optimal regret performance for strongly convex and separably nonsmooth functions. An interesting finding is that the optimal progression of precision across iterations is independent of the low-dimensional CM routine employed, suggesting a general framework for extending low-dimensional optimization routines to high-dimensional problems. The proposed algorithm is amenable to online implementation and inherits the scalability and parallelizability properties of CM for large-scale optimization. Requiring only a sublinear order of message exchanges, it also lends itself well to distributed computing as compared with the alternative approach of coordinate gradient descent.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


We considered stochastic convex optimization where an unknown stochastic loss function is minimized based on noisy estimates of partial (sub-)gradients. We have developed a framework based on coordinate/block minimization that approaches the global minimizer by moving successively along each coordinate.
Referred to as Progressive Coordinate Minimization (PCM),  the proposed framework consists of a global control module that prescribes the precision level in each CM iteration and a local low-dimensional stochastic optimization routine augmented with a self termination rule for stopping with the required precision. An interesting finding is that the optimal progression of precision across iterations is independent of the low-dimensional routine employed, suggesting a general framework for extending low-dimensional optimization routines to high-dimensional problems. The proposed algorithm is amenable to online implementation due to its low memory complexity and inherits the scalability and parallelizability  properties of CM for large-scale optimization problems. This appears to be the first study on generalizing CM approaches to stochastic optimization, which has the advantage of low communication overhead in distributed implementation as compared with the alternative approach of coordinate gradient descent. Future directions include extensions of PCM to general convex and non-convex objective functions.    
